Quality Diversity Through Surprise

Quality diversity is a recent family of evolutionary search algorithms which focus on finding several well-performing (quality) yet different (diversity) solutions with the aim to maintain an appropriate balance between divergence and convergence during search. While quality diversity has already delivered promising results in complex problems, the capacity of divergent search variants for quality diversity remains largely unexplored. Inspired by the notion of surprise as an effective driver of divergent search and its orthogonal nature to novelty this paper investigates the impact of the former to quality diversity performance. For that purpose we introduce three new quality diversity algorithms which employ surprise as a diversity measure, either on its own or combined with novelty, and compare their performance against novelty search with local competition, the state of the art quality diversity algorithm. The algorithms are tested in a robot navigation task across 60 highly deceptive mazes. Our findings suggest that allowing surprise and novelty to operate synergistically for divergence and in combination with local competition leads to quality diversity algorithms of significantly higher efficiency, speed and robustness.

==> fig_1.tex <==
\begin{figure*}[!tb]
\centering
\includegraphics[width=1\textwidth]{./graph/fig_1}
\caption{\textbf{Surprise-based Quality Diversity}. The flow chart illustrates a high level representation of the three introduced QD algorithms: SS-LC, NSS-LC, NS-SS-LC. All algorithms are based on a steady state evolutionary algorithm framework (left flow chart). The model of surprise is initialized after the generation of the initial population and then updated every $N$ offspring generations (right flow chart). The evaluation of individuals (middle flow chart) goes through the calculation of local competition, novelty, and surprise scores before those are assigned to the corresponding algorithm.
{The introduced surprise-based components and novelty-surprise components of the algorithm are depicted in grey boxes and in black boxes respectively.}
References are made to parts of existing divergent search and QD algorithms, as well as corresponding equations and sections in this paper.
}
\label{fig:qd_steady_state}
\end{figure*}

==> fig_2.tex <==
\begin{figure}[tb]
	\centering
	\subfloat[Generation $g - 2$]{
	\includegraphics[width=0.31\linewidth]{./graph/fig_2_a}}
	\subfloat[Generation $g - 1$]{
	\includegraphics[width=0.31\linewidth]{./graph/fig_2_b}}
    \subfloat[Generation $g$]{
    \includegraphics[width=0.31\linewidth]{./graph/fig_2_c}}
    \caption{The key phases of the surprise search algorithm as applied to the maze navigation domain. Surprise search uses a history of two generations ($h=2$) and 10 behavioral clusters ($k_{SS}=10$) in this example. Robots' final positions are depicted as empty squares; cluster centroids and prediction points are depicted as light grey and dark grey circles, respectively.}
    \label{fig:surprise_search}
\end{figure}

==> fig_3.tex <==
\begin{figure}[!tb]
    \centering
    \subfloat[Local competition $n_{LC}= 5$]{
    \includegraphics[width=0.48\linewidth]{graph/fig_3_a}
    \label{fig:sensitivity_lc_5}}
    \subfloat[Local competition $n_{LC}= 10$]{
    \includegraphics[width=0.48\linewidth]{graph/fig_3_b}
    \label{fig:sensitivity_lc_10}} 
    \\
    \subfloat[Local competition $n_{LC}= 15$]{
    \includegraphics[width=0.48\linewidth]{graph/fig_3_c}
    \label{fig:sensitivity_lc_15}}
    \subfloat[Local competition $n_{LC}= 20$]{
    \includegraphics[width=0.48\linewidth]{graph/fig_3_d}
    \label{fig:sensitivity_lc_20}}

\caption{\textbf{Sensitivity analysis:}
Average number of evaluations in the 10 easiest mazes across four local competition sizes (5, 10, 15, 20) and five values of $\lambda$ (0.4, 0.5, 0.6, 0.7, 0.8). Error bars denote 95\% confidence intervals.}
\label{fig:sensitivity}
\end{figure}

==> fig_4.tex <==
\begin{figure}[tb]
\centering
\includegraphics[height=0.55\linewidth]{graph/fig_4}
\caption{\textbf{Sensitivity to algorithmic components:} Average number of evaluations in the 10 easiest mazes across five QD approaches (NS-LC, NSS-LC, SS-LC, SSA-LC, NS-SS-LC) and four divergent search algorithms (NS, SS, NSS, NS-SS). Error bars denote 95\% confidence intervals.}
\label{fig:sensitivity_components}
\end{figure}

==> fig_5.tex <==
\begin{figure}[!tb]
		\centering
		\includegraphics[height=0.64\linewidth]{graph/fig_5}
		\caption{\textbf{Robustness:} number of successes over evaluations by aggregating all the runs across the 60 generated mazes for each approach.}
		\label{fig:robustness}
\end{figure}

==> fig_6.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[height=0.6\linewidth]{graph/fig_6}
\caption{\textbf{Average number of evaluations} from all the runs across the 60 generated mazes of each algorithm (i.e., 3000 runs per algorithm). Error bars denote 95\% confidence intervals.}
\label{fig:evaluations}
\end{figure}

==> fig_7.tex <==
\begin{figure}[tb]
\centering
\subfloat{\includegraphics[height=0.31\linewidth]{graph/fig_7_a}} 
\hfill
\subfloat{\includegraphics[height=0.31\linewidth]{graph/fig_7_b}}
\caption{\textbf{Complexity:} number of connections (left figure) and hidden nodes (right figure) on average for evolved ANNs which solve the mazes per approach. Error bars denote 95\% confidence intervals.}
\label{fig:complexity}
\end{figure}

==> table_1.tex <==

% 	\begin{figure}[tb]
% 		\captionsetup[subfigure]{justification=centering}
% 		\newcommand\maze{0.175}
% 		\centering
% 		\subfloat[][R = 8,\hspace{\textwidth} L = 453, \hspace{\textwidth}S = 50]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_a}\label{fig:maze_example_1}
% 		}
% 		\subfloat[][R = 8, \hspace{\textwidth} L = 332, \hspace{\textwidth}S = 40]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_b}\label{fig:maze_example_2}
% 		}
% 		\subfloat[][R = 6, \hspace{\textwidth} L = 362, \hspace{\textwidth}S = 32]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_c}\label{fig:maze_example_3}
% 		}
% 		\subfloat[][R = 6,\hspace{\textwidth} L = 391, \hspace{\textwidth}S = 22]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_d}\label{fig:maze_example_4}
% 		}
% 		\subfloat[][R = 8,\hspace{\textwidth} L = 364, \hspace{\textwidth}S = 17]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_e}\label{fig:maze_example_5}
% 		}
% 		\\
% 		\subfloat[][R = 6, \hspace{\textwidth}L = 333, \hspace{\textwidth}S = 16]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_f}\label{fig:maze_example_6}
% 		}
% 		\subfloat[][R = 9, \hspace{\textwidth}L = 355, \hspace{\textwidth}S = 15]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_g}\label{fig:maze_example_7}
% 		}
% 		\subfloat[][R = 11,  \hspace{\textwidth}L = 325, \hspace{\textwidth}S = 14]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_h}\label{fig:maze_example_8}
% 		}
% 		\subfloat[][R = 5, \hspace{\textwidth}L = 488, \hspace{\textwidth}S = 12]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_i}\label{fig:maze_example_9}
% 		}
% 		\subfloat[][R = 10, \hspace{\textwidth}L = 325, \hspace{\textwidth}S = 5]{
% 			\includegraphics[width=\maze\linewidth]{graph/mazes/fig_3_l}\label{fig:maze_example_10}
% 		}
% 		\caption{\textbf{Maze generation:} 10 easiest generated mazes %of 200x200 units 
% 		created via recursive division, sorted by NS-LC successes. The starting position (blue filled circle) is at the bottom left corner; the goal position (black empty circle) is at the top right corner. In the caption, R is the number of subdivisions, L is the A* length and S is the number of successes of NS-LC ($n_{LC} = 15$).}
% 		\label{fig:maze_example}
% 	\end{figure}
    
\begin{table}[!tb]
	
	\centering
	
	\caption{Ten easiest generated mazes sorted by NS-LC successes. 
    The starting position (grey filled circle) is at the bottom left corner; the goal position (black empty circle) is at the top right corner. The three numbers under each maze from left to right represent, respectively, the number of subdivisions, the A* path length, and the number of successes of NS-LC.}
    %$R$ is the number of subdivisions, $L$ is the A* length and $S$ is the number of successes of NS-LC.}
	\label{fig:maze_example}
	
	\bgroup
	
	\newcommand \size{0.155\linewidth}
   \newcommand\maze{1}
	
	\begin{tabular}{c c c c c}
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_a}} &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_b}} &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_c}} &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_d}} &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_e}}\\
%    $R = 8$ &
%    $R = 8$ & 
%    $R = 6$ & 
%    $R = 6$ & 
%    $R = 8$ \\
%    $L = 453$ &
%    $L = 332$ & 
%    $L = 362$ & 
%    $L = 391$ & 
%    $L = 364$ \\
%    $S = 50$ &
%    $S = 40$ & 
%    $S = 32$ & 
%    $S = 22$ & 
%    $S = 17$ \\
 $\left[8, 453, 50\right]$ & $\left[8, 332, 40\right]$ & $\left[6, 362, 32\right]$ & $\left[6, 391, 22\right]$ & $\left[8, 364, 17\right]$ \\ 
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_f}}  &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_g}}  &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_h}}  &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_i}} &
    \parbox[c][\size]{\size}{\includegraphics[width=\maze\linewidth]{graph/mazes/tab_1_l}} \\
%    $R = 6$ &
%    $R = 9$ & 
%    $R = 11$ & 
%    $R = 5$ & 
%    $R = 10$ \\
%    $L = 333$ &
%    $L = 355$ & 
%    $L = 325$ & 
%    $L = 488$ & 
%    $L = 325$ \\
%    $S = 16$ &
%    $S = 15$ & 
%    $S = 14$ & 
%    $S = 12$ & 
%    $S = 5$ \\
$\left[6, 333, 16\right]$ & $\left[9, 355, 15\right]$ & $\left[11, 325, 14\right]$ & $\left[5, 488, 12\right]$ & $\left[10, 325, 5\right]$ \\
    \end{tabular}
	\egroup
\end{table}
		

==> table_2.tex <==
\begin{table}[tb]
\centering
\caption{Distribution of the 60 selected mazes and corresponding average length of their shortest path, as computed by A*, across the number of subdivisions.}
\begin{tabular}{l||@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }}
\hline\hline
Subdivisions & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
\hline
Number of Mazes & 2 & 9 & 5 & 16 & 13 & 10 & 4 & 1 \\ 
A* length &  403 & 350 & 358 & 353 & 330 & 318 & 323 & 291 \\
\hline\hline
\end{tabular}
\label{tab:maze_stats}
\end{table}

==> table_3.tex <==
\begin{table}
\centering
\caption{Chosen parameters for QD algorithms based on a sensitivity analysis, and the average number of evaluations (with 95\% confidence intervals) obtained on the mazes of Fig.~\ref{fig:maze_example}.}
\label{tab:final_parameters}
\begin{tabular}{l||p{3.9cm}l}
\hline\hline
Algorithm & Parameters & Evaluations (${\cdot}10^3$) \\ \hline\hline
NS-LC & $n_{LC}=5$, $n_{NS}=15$ & $109.8 \pm 4.4$ \\ \hline
\multirow{2}{*}{SS-LC} & $n_{LC}=10$, $n_{SS}=2$,  & \multirow{2}{*}{$115.7 \pm 4.0$}\\ 
& $h=2$, $k_{SS}=200$  & \\ \hline
\multirow{2}{*}{NSS-LC} & $\lambda=0.7$, $n_{LC}=5$, $n_{NS}=15$, & \multirow{2}{*}{$104.2 \pm 4.5$} \\ 
&  $n_{SS}=2$, $h=2$, $k_{SS}=200$ & \\ \hline
\multirow{2}{*}{NS-SS-LC} & $n_{LC}=5$, $n_{NS}=15$, $n_{SS}=2$, & \multirow{2}{*}{$111.0 \pm 4.2$} \\ 
& $h=2$, $k_{SS}=200$ & \\ \hline\hline
\end{tabular}
\end{table}

==> table_4.tex <==
\begin{table}[!tb]
\centering
\caption{Algorithms tournament: Percentage of 60 generated mazes for which the algorithm in a row has a strictly greater (${\geq}1$)  number of successes compared to the algorithm in a column. Last row and last column are respectively the average of each column and the average of each row.}\label{table:rankings}
\begin{tabular}{l@{ }||@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }||@{ }c@{ }}
\hline\hline    
& NS & NS-LC & NSS-LC & SS-LC & NS-SS-LC &  Average    \\
\hline \hline     
NS & -- & 1.7\% & 0.0\% & 5.0\% & 1.7\% & 2.1\% \\ \hline
NS-LC & 83.3\% & -- & 30.0\% & 51.7\% & 40.0\% & 51.2\% \\ \hline
NSS-LC & 81.7\% & 48.3\% & -- & 60.0\% & 45.0\% & 58.7\% \\ \hline
SS-LC & 70.0\% & 28.3\% & 25.0\% & -- & 30.0\% & 38.3\% \\ \hline
NS-SS-LC & 80.0\% & 41.7\% & 26.7\% & 46.7\% & -- & 48.7\% \\
\hline \hline					
Average & 78.7\% & 30.0\% & 20.4\% & 40.8\% & 29.2\% & -- \\
\hline\hline
\end{tabular}
\label{tab:tournament_successes}
\end{table}
